See What the Robot Can't See: Learning Cooperative Perception for Visual Navigation

We consider the problem of navigating a mobile robot towards a target in an unknown environment that is endowed with visual sensors, where neither the robot nor the sensors have access to global positioning information and only use first-person-view images. In order to overcome the need for positioning, we train the sensors to encode and communicate relevant viewpoint information to the mobile robot, whose objective it is to use this information to navigate to the target along the shortest path. We overcome the challenge of enabling all the sensors (even those that cannot directly see the target) to predict the direction along the shortest path to the target by implementing a neighborhood-based feature aggregation module using a Graph Neural Network (GNN) architecture. In our experiments, we first demonstrate generalizability to previously unseen environments with various sensor layouts. Our results show that by using communication between the sensors and the robot, we achieve up to 2.0x improvement in SPL (Success weighted by Path Length) when compared to a communication-free baseline. This is done without requiring a global map, positioning data, nor pre-calibration of the sensor network. Second, we perform a zero-shot transfer of our model from simulation to the real world. Laboratory experiments demonstrate the feasibility of our approach in various cluttered environments. Finally, we showcase examples of successful navigation to the target while both the sensor network layout as well as obstacles are dynamically reconfigured as the robot navigates. We provide a video demo, the dataset, trained models, and source code. https://www.youtube.com/watch?v=kcmr6RUgucw https://github.com/proroklab/sensor-guided-visual-nav

==> Figs/sim_to_real/tikzset.tex <==
\tikzset{
    enc/.style = {minimum width=3cm, minimum height=1.9em, trapezium, trapezium angle=-75, draw, trapezium stretches=true, inner sep=0.4em},
    node_label/.style = {inner sep=0.4em},
    block/.style = {draw=black, inner sep=0.4em},
    sim/.style = {fill=orange!30},
    real/.style = {fill=gray!30},
    comm/.style = {decorate,decoration={snake, amplitude=0.4mm, segment length=3mm, post length=1mm}},
}


==> format/glossary.tex <==
\newacronym{AGNN}{AGNN}{Aggregation Graph Neural Network}
\newacronym{RL}{RL}{Reinforcement Learning}
\newacronym[longplural={Markov Decision Processes}]{MDP}{MDP}{Markov Decision Process}
\newacronym[longplural={Partially Observable Markov Decision Processes}]{POMDP}{POMDP}{Partially Observable Markov Decision Process}
\newacronym[longplural={Decentralized Partially Observable Markov Decision Processes}]{DecPOMDP}{Dec-POMDP}{Decentralized POMDP}
\newacronym{NN}{NN}{Neural Network}
\newacronym{CNN}{CNN}{Convolutional Neural Network}
\newacronym{GSO}{GSO}{Graph Shift Operator}
\newacronym{GPS}{GPS}{Global Positioning System}
\newacronym{GNN}{GNN}{Graph Neural Network}
\newacronym{PBT}{PBT}{Population Based Training}
\newacronym{PG}{PG}{Policy Gradient}
\newacronym{MLP}{MLP}{Multi Layer Perceptron}
\newacronym{LSTM}{LSTM}{Long Short-term Memory}
\newacronym{PPO}{PPO}{Proximal Policy Optimization}
\newacronym{mAP}{mAP}{mean Average Precision}
\newacronym{TRPO}{TRPO}{Trust Region Policy Optimization}
\newacronym{MARL}{MARL}{Multi-Agent Reinforcement Learning}
\newacronym{DQN}{DQN}{Deep Q-Learning}
\newacronym{GCNN}{GCNN}{Graph Convolutional Neural Network}
\newacronym{CPP}{CPP}{Coverage Path Planning}
\newacronym{VPG}{VPG}{Vanilla Policy Gradient}

\glsdisablehyper % no hyperrefs in glossary


==> format/math_defns.tex <==
%%%%%%%%%%%%%%%%General Purpose %%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%% Graph Defns %%%%%%%%%%%%%%%%%%%%%
\newcommand{\Graph}[0]{G}
\newcommand{\vertexSet}[0]{V}
\newcommand{\edgeSet}[0]{E}
\newcommand{\invalidEdgeSet}{\edgeSet_\mathrm{invalid}}
\newcommand{\vertex}[0]{v}
\newcommand{\edge}[0]{e}
\newcommand{\start}[0]{v_s}
\newcommand{\goal}[0]{v_g}
\newcommand{\succFnDef}[0]{\mathtt{Succ}}
\newcommand{\succFn}[1]{\succFnDef(#1)}
\newcommand{\Path}[0]{\xi}
\newcommand{\PathSet}[0]{\Xi}
\newcommand{\evalFn}[0]{\mathtt{Eval}}
\newcommand{\edgeCost}[0]{C(\edge)}



%%%%%%%%%%%%%%%%%%%%% Planner Defns %%%%%%%%%%%%%%%%%%%%%
\newcommand{\plannerTuple}[6]{\langle#1, #2, #3, #4, #5, #6\rangle}
\newcommand{\state}[0]{s}
\newcommand{\action}[0]{a}
\newcommand{\obs}[0]{o}
\newcommand{\search}[0]{\mathtt{Search}}
\newcommand{\select}[0]{\mathtt{Select}}
\newcommand{\expand}[0]{\mathtt{Expand}}

\newcommand{\vertexSucc}[0]{V_\mathrm{succ}}
\newcommand{\invalidEdge}[0]{E_\mathrm{inv}}


\newcommand{\searchState}{\{\openList, \closedList, \closedObsList \}}
%\newcommand{\searchStatet}[0]{\langle \openList_t, \closedList_t, \closedObsList_{t}, \unexploredList_t \rangle}
\newcommand{\stateSpace}{\mathcal{S}}
\newcommand{\actionSpace}{\mathcal{A}}
\newcommand{\openList}[0]{\mathcal{O}}
\newcommand{\closedList}[0]{\mathcal{C}}
\newcommand{\closedObsList}[0]{\mathcal{I}}
\newcommand{\unexploredList}[0]{\mathcal{U}}
\newcommand{\priorityFn}[2]{\mathtt{Pr\pair{#1}{#2}}}
%\newcommand{\actionGivenState}[0]{\action|\state}
%\newcommand{\actionGivenSearchState}[0]{\action|\searchState}
%\newcommand{\actionGivenOpen}[0]{\action|\openList}
\newcommand{\planTime}[0]{T}
%%%%%%%%%%%%%%%%%%%%% Policy Defns %%%%%%%%%%%%%%%%%%%%%
\newcommand{\policy}[0]{\pi}
\newcommand{\policySpace}[0]{\Pi}
\newcommand{\policyOpt}[0]{\policy^*}
\newcommand{\policyLearn}[0]{\hat{\policy}}
\newcommand{\policyMix}[0]{\policy_\mathrm{mix}}
\newcommand{\policyOracle}[0]{\policy_\mathrm{OR}}
\newcommand{\policyOracleBel}[0]{\tilde{\policy}_\mathrm{OR}}
\newcommand{\policyGreedy}[0]{\policy_\mathrm{greedy}}
\newcommand{\costToGopolicy}[1]{Q_{t}^{#1}}
\newcommand{\costToGoOracle}{Q^{\textsc{COR}}}
\newcommand{\costToGo}{Q}
\newcommand{\lossFn}{\mathcal{L}}
%%%%%%%%%%%%%%%%%%%%% MDP Defns %%%%%%%%%%%%%%%%%%%%%
\newcommand{\world}[0]{\phi}
\newcommand{\belief}[0]{\psi}
\newcommand{\worldSet}[0]{\mathcal{M}}
\newcommand{\worldProb}[0]{\prob{\world}}
\newcommand{\measurementFn}[2]{\mathcal{H}\pair{#1}{#2}}
\newcommand{\history}[0]{\left\{(\state_t, \action_t, \obs_t)\right\}_{i=1}^{t}}
\newcommand{\costonestep}[0]{c}
\newcommand{\cost}[0]{J}
\newcommand{\startProb}[0]{\prob{\start,\goal}}
\newcommand{\timeAvgDist}[0]{d_{\policy}^{t}}
\newcommand{\featureFunc}{\textsc{f}}
\newcommand{\featureVec}{f}
\newcommand{\featureSpace}{\mathcal{F}}
%%%%%%%%%%%%%%%%% Algorithm Defns %%%%%%%%%%%%%%%%%%%%
\newcommand{\dataset}[0]{\mathcal{D}}
\newcommand{\thetaLearn}[0]{\hat{\theta}}
\newcommand{\thetaSpace}[0]{\Theta}
\newcommand{\mixParam}[0]{\beta}
\newcommand{\dataPointsParam}{k}
\newcommand{\errclass}[0]{\varepsilon_{\mathrm{class}}}
\newcommand{\errreg}[0]{\varepsilon_{\mathrm{reg}}}

%%%%%%%%%%%%%%%%% Experiment Defns %%%%%%%%%%%%%%%%%%%%
\newcommand{\greedyEuc}{h_{\textsc{EUC}}}
\newcommand{\greedyMan}{h_{\textsc{MAN}}}
\newcommand{\distObs}{d_{OBS}}
\newcommand{\policyEuc}{\policy_{\textsc{EUC}}}
\newcommand{\policyMan}{\policy_{\textsc{MAN}}}
\newcommand{\gVal}{g_{\vertex}}
\newcommand{\treeDepth}{d_{TREE}}


\newcommand{\rulesep}{\unskip\ \vrule\ }





\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

\newcommand{\new}[1]{\emph{#1}}
\newcommand{\cA}{\ensuremath{{\mathcal A}}\xspace}
\newcommand{\cB}{\ensuremath{{\mathcal B}}\xspace}
\newcommand{\cC}{\ensuremath{{\mathcal C}}\xspace}
\newcommand{\cD}{\ensuremath{{\mathcal D}}\xspace}
\newcommand{\cF}{\ensuremath{{\mathcal F}}\xspace}
\newcommand{\cH}{\ensuremath{{\mathcal H}}\xspace}
\newcommand{\cN}{\ensuremath{{\mathcal N}}\xspace}
\newcommand{\cO}{\ensuremath{{\mathcal O}}\xspace}
\newcommand{\cP}{\ensuremath{{\mathcal P}}\xspace}
\newcommand{\cR}{\ensuremath{{\mathcal R}}\xspace}
\newcommand{\cS}{\ensuremath{{\mathcal S}}\xspace}
\newcommand{\cU}{\ensuremath{{\mathcal U}}\xspace}
\newcommand{\cV}{\ensuremath{{\mathcal V}}\xspace}
\newcommand{\cPn}{\ensuremath{{\mathcal P}_n}\xspace}

\newcommand{\fA}{\ensuremath{\mathfrak{A}}\xspace}
\newcommand{\fB}{\ensuremath{\mathfrak{B}}\xspace}
\newcommand{\fC}{\ensuremath{\mathfrak{C}}\xspace}

\newcommand{\fa}{\ensuremath{\mathfrak{a}}\xspace}
\newcommand{\fb}{\ensuremath{\mathfrak{b}}\xspace}
\newcommand{\fc}{\ensuremath{\mathfrak{c}}\xspace}
\newcommand{\fd}{\ensuremath{\mathfrak{d}}\xspace}

\newcommand{\bA}{\ensuremath{{\bf A}}\xspace}
\newcommand{\bB}{\ensuremath{{\bf B}}\xspace}
\newcommand{\bK}{\ensuremath{{\bf K}}\xspace}
\newcommand{\bE}{\ensuremath{{\bf E}}\xspace}
\newcommand{\bN}{\ensuremath{{\bf N}}\xspace}
\newcommand{\bG}{\ensuremath{{\bf G}}\xspace}

\newcommand{\ba}{\ensuremath{{\bf a}}\xspace}
\newcommand{\bb}{\ensuremath{{\bf b}}\xspace}
\newcommand{\bc}{\ensuremath{{\bf c}}\xspace}

\newcommand{\bbE}{\ensuremath{\mathbb{E}}}
\newcommand{\bbR}{\ensuremath{\mathbb{R}}}
\newcommand{\bbQ}{\ensuremath{\mathbb{Q}}}
\newcommand{\bbP}{\ensuremath{\mathbb{P}}}
\newcommand{\bbZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\bbN}{\ensuremath{\mathbb{N}}}
\newcommand{\bbNn}{\ensuremath{\mathbb{N}_0}}

\newcommand{\bbRnp}{\ensuremath{\bbR_{\geq 0}}}
\newcommand{\bbQnp}{\ensuremath{\bbQ_{\geq}}}
\newcommand{\bbZnp}{\ensuremath{\bbZ_{\geq}}}

\newcommand{\bbRsp}{\ensuremath{\bbR_>}}
\newcommand{\bbQsp}{\ensuremath{\bbQ_>}}
\newcommand{\bbZsp}{\ensuremath{\bbZ_>}}

\newcommand{\cp}{\textsf{P}\xspace}
\newcommand{\cnp}{\textsf{NP}\xspace}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\GN}{\mathbb{G}_n}

\newcommand{\rb}{\right\}\xspace}
\newcommand{\lb}{\left\{\xspace}
\newcommand{\lbr}{\left(\xspace}
\newcommand{\rbr}{\right)\xspace}

\newcommand{\trans}{^T}
\renewcommand{\vec}[1]{\mathbf{#1}} %TODO: avoid renewcommand!

\newcommand{\oms}{\{\!\!\{}
\newcommand{\cms}{\}\!\!\}}

\newcommand{\cl}{\operatorname{cl}}
\newcommand{\rk}{\operatorname{rk}}
\newcommand{\sgn}{\operatorname{sgn}}




















%%%%%%%%%%%%%%%%% DRD BERN Defns %%%%%%%%%%%%%%%%%%%%
%
%\newcommand{\test}[0]{t}
%\newcommand{\testSet}[0]{\mathcal{T}}
%\newcommand{\numTest}[0]{n}
%
%\newcommand{\outcomeSpace}[0]{\{0, 1\}}
%\newcommand{\outcomeVar}[0]{X}
%\newcommand{\outcomeVarTest}[1]{\outcomeVar_{#1}}
%\newcommand{\outcome}[0]{x}
%\newcommand{\outcomeTest}[1]{\outcome_{#1}}
%\newcommand{\outcomeTestSet}[1]{\mathbf{\outcome}_{#1}}
%
%\newcommand{\bias}[0]{\theta}
%\newcommand{\biasVec}[0]{\bm{\bias}}
%\newcommand{\biasTest}[1]{\bias_{#1}}
%
%\newcommand{\region}[0]{\mathcal{R}}
%\newcommand{\numRegion}[0]{m}
%\newcommand{\nullRegion}[0]{\mathcal{R}_0}
%
%\newcommand{\selTestSet}[0]{\mathcal{A}}
%\newcommand{\obsOutcome}[0]{\outcomeTestSet{\selTestSet}}
%\newcommand{\obsOutcomeFunc}[2]{\obsOutcome \left( #1, #2\right)}
%\newcommand{\obsOutcomeAdd}[1]{\outcomeTestSet{\selTestSet \cup \set{#1}}}
%
%
%\newcommand{\policy}[0]{\pi}
%\newcommand{\groundtruth}[0]{\outcomeTestSet{\testSet}}
%
%\newcommand{\cost}[0]{c}
%\newcommand{\policyOpt}[0]{\pi^*}
%
%
%%%%%%%%%%%%%%% EC2 %%%%%%%%%%%%%%%%%%%
%\newcommand{\hyp}[0]{h}
%\newcommand{\hypSpace}[0]{\mathcal{H}}
%\newcommand{\hypSpaceR}[0]{\mathcal{H}^\region}
%\newcommand{\regionH}[0]{\region^\hypSpace}
%
%
%\newcommand{\subregion}[0]{\mathcal{S}}
%\newcommand{\numSubregion}[0]{l}
%
%\newcommand{\edgeEC}[0]{\varepsilon}
%\newcommand{\edgeSetEC}[0]{\mathcal{E}}
%\newcommand{\edgeFnEC}[2]{\{#1, #2\}}
%
%\newcommand{\weight}[0]{w}
%
%\newcommand{\ec}[0]{f_\mathrm{EC}}
%\newcommand{\fec}[1]{f_\mathrm{EC}(#1)}
%\newcommand{\ecgolovin}[0]{f_{\text{\citep{golovin2010near}}}}
%\newcommand{\gain}[3]{\Delta_{#1} \left( #2 \;|\; #3 \right)}
%
%\newcommand{\wec}[0]{w_\mathrm{EC}}
%\newcommand{\wecgolovin}[0]{w_{\text{\citep{golovin2010near}}}}
%
%
%\newcommand{\ectext}[0]{\mathrm{EC}}
%\newcommand{\drd}[0]{f_\mathrm{DRD}}
%\newcommand{\fdrd}[1]{f_\mathrm{DRD}(#1)}
%\newcommand{\feci}[2]{f_\mathrm{EC}^{#1}(#2)}
%
%%%%% Algorithm
%\newcommand{\candTestSet}[0]{\testSet_\mathrm{cand}}
%\newcommand{\optTest}[0]{t^*}
%\newcommand{\maxProbTestSet}[0]{\testSet_\mathrm{maxP}}
%
%\newcommand{\aliveRegionSet}[0]{\region_\mathrm{alive}}
%
%%%%% Lattice
%\newcommand{\degree}[0]{k}
%
%\newcommand{\nv}[0]{n_\mathcal{V}}
%\newcommand{\nvec}[0]{\mathbf{n}}
%
%%%% Suboptimal
%\newcommand{\pmin}[0]{p_\mathrm{min}}
%\newcommand{\pminH}[0]{p_\mathrm{min}^h}
%
%\newcommand{\dataTrain}[0]{N_{\mathrm{train}}}
%\newcommand{\dataTest}[0]{N_{\mathrm{test}}}
%%% Synthetic bernoulli
%\newcommand{\regTest}[0]{\mathbf{A}}
%
%
%%%% runtime
\newcommand{\bigo}[1]{\mathcal{O}\left(#1\right)}


==> format/text_shortcuts.tex <==
\newcommand{\daggerAlg}[0]{\textsc{DAgger}}
\newcommand{\aggravateAlg}[0]{\textsc{AggreVaTe}}
\newcommand{\algName}[0]{\textsc{SaIL}\xspace}
\newcommand{\algFullName}[0]{Search as Imitation Learning \xspace}
%
%
%\newcommand{\algRandom}[0]{\textsc{Random}\xspace}
%\newcommand{\algMaxTally}[0]{\textsc{MaxTally}\xspace}
%\newcommand{\algSetCover}[0]{\textsc{SetCover}\xspace}
%\newcommand{\algMVOI}[0]{\textsc{MVoI}\xspace}
%
%\newcommand{\probBernDRD}[0]{Bern-DRD\xspace}
%\newcommand{\probBernDRDFull}[0]{decision region determination with independent Bernoulli tests\xspace}
%
%\newcommand{\algMaxProbReg}[0]{\textsc{MaxProbReg}\xspace}

